Design and Evaluation of a Tutor Platform for Personalized Vocabulary Learning

This paper presents our experiences in designing, implementing, and piloting an intelligent vocabulary learning tutor. The design builds on several intelligent tutoring design concepts, including graph-based knowledge representation, learner modeling, and adaptive learning content and assessment exposition. Specifically, we design a novel phased learner model approach to enable systematic exposure to words during vocabulary instruction. We also built an example application over the tutor platform that uses a learning activity involving videos and an assessment activity involving word to picture/image association. More importantly, the tutor adapts to the significant variation in children's knowledge at the beginning of kindergarten, and evolves the application at the speed of each individual learner. A pilot study with 180 kindergarten learners allowed the tutor to collect various kinds of activity information suitable for insights and interventions both at an individual- and class-level. The effort also demonstrates that we can do A/B testing for a variety of hypotheses at scale with such a framework.

==> eval.tex <==
\section{Experimental Evaluation}
\label{sec:evaluation}

In this section, we discuss an application built on the tutor that exposes videos for learning, and tests receptive vocabulary via word to picture mapping/association. An experimental study was conducted to evaluate the efficacy of this application built for early-childhood vocabulary learning.

\subsection{Methodology}
Since the effectiveness of the application requires causal claims for evaluation, an intervention study is needed. The pilot study was conducted during a 9-week period at Gwinnett County Public Schools (GCPS) between October and December 2017. In the following, we describe the data collection, the A/B testing setup, and the metrics used for evaluation.

\subsubsection{Data and Participants}
\label{sec:data}
%About GCPS, classrooms, age groups, and other stats.
The data was collected using an application that presents videos built around explaining the word concept. They are used as interventions or learning activities and are decided for a learner based on their learner model in the tutor. The learner model in the tutor was in turn updated using multiple-choice assessments that test receptive vocabulary via word to picture mapping/association. As per the discussion in Sec.~\ref{sec:tutor-arch}, this particular application built in the experience layer of the tutor, is updating the learner score in listening comprehension dimension, and was presented to the learner using predominantly vision and touch interactions. Each assessment question had the test word spoken aloud followed by three images to choose from. While the learner was given two chances to pick the relevant image, the response was considered to be correct only if it was correct in the first attempt itself. Fig.~\ref{fig:WC} shows an example assessment.

\begin{figure}
\centering
\includegraphics[width = 3in, height=!]{WC.png}
\caption{An example assessment question.}
\label{fig:WC}
\end{figure}

For this study, we focused on $N=181$ early-kindergarten learners from $8$ classes across $4$ public schools in north central portion of the state of Georgia, USA. The application focused on $K=40$ vocabulary words that have been picked by subject matter experts as target words to be taught to the learners.

\subsubsection{A/B Testing}
It is important to note that the application's success could depend on the concept/vocabulary word of focus. In order to collect data for all the words while including every learner in the experimental group, we designed the A/B testing methodology in the following manner: the classrooms were randomly split into two groups (Group A and Group B), with all learners within a class belonging to the same group. Similarly all vocabulary words were divided into two word sets (Word Set $X$ and Word Set $Y$). For Group A learners, learning activity was available only on word set $X$, while they were assessed on both word sets $X$ and $Y$. Similarly, Group B learners had learning activity only for word set $Y$, while they were assessed on both word sets $X$ and $Y$. In this way, for words in word set $X$, Group A learners acted as the experimental group and Group B learners were the control group. And for words in word set $Y$, Group B learners acted as the experimental group and Group A learners were the control group. This ensured that every learner belonged to the experimental group and took part in learning activities for some subset of vocabulary words. These learning activities were \textbf{x minute long} videos describing the word, developed by Sesame Workshop. Table~\ref{table:AB} summarizes the A/B testing methodology.

\begin{table}
\begin{center}
\caption{A/B Testing Methodology}
\begin{tabular}{|c||c|c|}
\hline
 & Group A & Group B\\
\hline
\hline
Number of classes &4 & 4\\
\hline
Number of learners &91 & 90\\
\hline
Learning activity & Word set $X$ & Word set $Y$\\
\hline
Assessment activity & Word set $X\cup Y$ & Word set $X\cup Y$\\
\hline
\end{tabular}
\end{center}
\label{table:AB}
\end{table}

\subsubsection{Metrics}
\label{sec:model}
The assessment responses from the application were used to evaluate the application's tutoring efficacy. The collected data is analyzed based on the following model. Let there be two sets of assessment response data ($G_1$ and $G_2$) each consisting of multiple assessment response vectors ($N_1$ vectors in $G_1$ and $N_2$ in $G_2$). For vector $l$ where $l=1,\ldots,N_1$, let $\mathbf{a}_l\in\{0,1\}^{t_l}$ be the $t_l$-length bit sequence representing the assessment responses.\footnote{$a_l$=1 if the assessment response is correct and $0$ otherwise.} %A single such assessment response sequence can be split into two shorter length sequences $\mathbf{y}_k\in\{0,1\}^{s_k}$ and $\mathbf{z}_k\in\{0,1\}^{t_k}$ with $s_k+t_k=l_k$, which are the pre-learning assessment sequence and the post-learning assessment sequence, respectively.
 
The goal is to determine if the data vectors in $G_2$ are ``significantly better" than the data vectors in $G_1$. In other words, the distribution of data in $G_2$ is ``significantly greater" than the distribution of data in $G_1$. This can be modeled as the following one-sided hypothesis test.
\begin{eqnarray}
H_0: f_\mathbf{G_1}=f_\mathbf{G_2}\nn\\
H_1: f_\mathbf{G_1}<f_\mathbf{G_2}
\label{eq:hyp_gen}
\end{eqnarray}
where $<$ is defined in the sense that the data values in $G_1$ tend to be \emph{larger} than those in $G_2$, or in other words the cumulative distribution function of $G_1$ tends to be smaller than that of $G_2$. These kind of statistical hypothesis tests help us evaluate the success or failure of tutoring interventions. 

Note that in such a general formulation, each data vector $\mathbf{a}_l$ can be of different length. Hence, determining the distribution of the vectors within the group is not straightforward. To address this concern, we make the following simplification: for each assessment response sequence $\mathbf{a}_l$, the assessment responses can be considered to be independently and identically distributed binary random variables and hence, the mean $p_l$ of $\mathbf{a}_l$ is the sufficient statistic to represent $\mathbf{a}_l$. Note that this assumption is a valid one especially when the underlying unknown distribution is Bernoulli distributed. 
Based on this discussion, \eqref{eq:hyp_gen} simplifies to testing if data $\mathbf{p}_1=[p_1,\ldots,p_{N_1}]$ and data $\mathbf{p}_2=[p_1,\ldots,p_{N_2}]$ come from significantly different distributions. In other words
\begin{eqnarray}
H_0: f_{\mathbf{p}_1}=f_{\mathbf{p}_2}\nn\\
H_1: f_{\mathbf{p}_1}<f_{\mathbf{p}_2}.
\label{eq:hyp_pq}
\end{eqnarray}
 
This test can be performed either using the one-sided two-sample t-test of means \cite{ChakravartyRL1967} which works well when the data is normally distributed or using the stricter one-sided two-sample Kolmogorov-Smirnov (KS) test \cite{ChakravartyRL1967}. The KS test is a goodness-of-fit test that works very well for continuous variables \cite{ChakravartyRL1967}.
Note that, the assessment sequence $\mathbf{a}_l$ is abstracted using mean $p_l$. To ensure statistical significance, we only consider the assessment vectors in $G_1$ and $G_2$ for which $t_l\geq\tau$. Also, while comparing distributions of $\mathbf{p}_1$ and $\mathbf{p}_2$, we need to ensure there is a lower limit $\eta$ on the size of $G_1$ and $G_2$. In other words, the analysis is performed only when $N_1\geq\eta$ and $N_2\geq\eta$.

\subsection{Research Questions and Hypotheses}
\label{sec:hyp}
%In this paper, our goal is to test the efficacy of the vocabulary tutor. The efficacy of any tutor is determined by comparing the performance of students with and without using the tutor. In this paper, we focus on the following two hypotheses using real learner data.

The vocabulary learning application built on the early vocabulary tutoring platform described above is oriented towards addressing the 30 million word gap. We determine the efficacy of the application by answering two fundamental research questions using the data. 

\paragraph*{Hypothesis 1:}
\label{hyp:1}
Learners' assessment performance (as evaluated by the application) after exposure to the tutor recommended learning activity, is higher than before the exposure to the learning activity.

Hypothesis 1 argues that learners perform better after intervention in comparison to before the tutor-powered application interventions. 

\paragraph*{Hypothesis 2:}
\label{hyp:2}
Performance of learners using the application built on the tutor is higher than the learners who do not use it.

Hypothesis 2 argues that the performance of learners with tutor-powered application interventions is better than the performance of learners without them. 

Both these questions can be answered using the data collected by appropriately modeling them using (\ref{eq:hyp_pq}). The results corresponding to these hypotheses are presented in the following. 

\subsection{Results}
In this section, we present the results obtained from the pilot study. For the study, the parameter values of the tutoring system used are summarized in Table~\ref{table:parameters}.

% "exponentialMovingAverageAlpha" : 0.8,
%   "numberOfAttemptsWindowSize": 3,
%   "minWorkingsetSize": 4,
%   "toLearnedPhaseValue": 0.86,
%   "outOfLearnedPhaseValue": 0.56,
%   "defaultVocabLearningScore" : 0.0001,
%   "defaultNonTargetVocabLearningScore" : 1,
%   "level1BlendLearnedWorkingsetParkedValues": "50,30,20",
%   "averageAssessmentWordsPerMin": 10,
%   "averageLearningTimeToMasterWordInMins": 10,

\begin{table}
\begin{center}
\caption{\label{table:parameters}Parameter values for experimental evaluation.}
\begin{tabular}{|l|c|}
\hline
Parameter & Value\\
\hline
EWMA parameter ($\alpha$) & 0.8\\
\hline
Threshold to transition into Learned Phase ($\tau_1=\tau_2$) & 0.86\\
\hline
Threshold to transition out of Learned Phase ($\tau_3=\tau_4$) & 0.56\\
\hline
% Minimum number of assessments before word moves to Working Set & 3\\
% \hline
$\tau$ & 3\\
\hline
$\eta$ & 10\\
\hline
\end{tabular}
\newline
\newline $\tau$ - minimum number of assessment responses needed
\newline $\eta$ - minimum number of learners needed in each of the groups
\end{center}
\end{table}

\subsubsection{General observations}
Before looking at the comparison results, it is worth making some general observations based on the pilot study. It is common knowledge that every learner is different and learns at a different pace. Fig.~\ref{fig:learningrate} shows a count of words with a high learning score over time for $5$ randomly picked learners. The plot shows that while all learners started with the same unknown confidence and low number of words with a high learning score, the pace of learning is different for every learner. This shows the need for personalization and the importance of one-on-one learning at scale which is now made possible by AI-powered tutoring systems. 

As mentioned before, the application built on the tutoring system has two major activities: learning activities, in the form of vocabulary words educational videos, and assessment activities, in the form of games, designed to assess the understanding of the word-image acquisition of the learner. To ensure that the learner does not completely avoid the assessment games, the application had a mechanism to trigger the need for an assessment if the learner did not spend a sufficient amount of time in assessment games. Fig.~\ref{fig:WC_likeness} plots the number of voluntary and total assessment games undertaken by individual learners. This shows the difference in likeness towards assessments for individual learners. From Figs.~\ref{fig:learningrate} and ~\ref{fig:WC_likeness}, it is clear that learners are unique across their learning rate and interests, strengthening the need for a personalized and adaptive tutor at scale.

\begin{figure}[t]
\begin{center}
	\subfigure[]{
	\includegraphics[width=0.475\textwidth]{LearningRate.png}\vspace{-0.2in}
	\label{fig:learningrate}	
	}
	\subfigure[]{
		\includegraphics[width=0.475\textwidth]{WC_likeness.png}\vspace{-0.2in}
		\label{fig:WC_likeness}
		}
\caption{\subref{fig:learningrate} Learning rates for different users. \subref{fig:WC_likeness} Assessment likeness for different users.\textbf{Change figure to say assessment likeness}}
%\label{fig:assessments}
\end{center}
\vspace{-0.3in}
\end{figure}

% \begin{figure}
% \centering
% \includegraphics[width = 3.5in, height=!]{ActivityPattern.png}
% \caption{Activity patterns for different users.}
% \label{fig:activity_pattern}
% \end{figure}

\subsubsection{Hypothesis 1}
We now try to answer the research question 1 of Sec.~\ref{sec:hyp}. The first hypothesis states that the performance of learners on the listening comprehension dimension as tested by the word-image association questions, is improved post the first learning activity, in comparison to before the learning activity. To answer this question, we set $G_1$ to be the set of assessment responses of all learners and words before the first learning activity, and $G_2$ to be the set of assessment responses of all learners and words after the learning activity. 

Based on the parameters used in Table~\ref{table:parameters}, the following results have been obtained. Fig.~\ref{fig:hyp1} shows the distribution of learners' performance in $G_1$ and $G_2$, i.e., before and after the first learning activity. From the figure, we can observe that there are more learners with a higher average correct responses after learning activity than before the first learning activity. More specifically, majority of the learners give correct responses 40-60\% of the times before any learning activity. On the other hand, after the first learning activity, majority of learners have provided correct responses 80-100\% of the times showing an increase in learner performance over time. 

\begin{figure}[t]
\begin{center}
	\subfigure[]{
	\includegraphics[width=0.425\textwidth]{Hyp1_fig.png}\vspace{-0.2in}
	\label{fig:hyp1}	
	}
	\subfigure[]{
		\includegraphics[width=0.525\textwidth, height = 1.35in]{Hyp1_Fig2.png}\vspace{-0.2in}
		\label{fig:hyp1_2}
		}
\caption{\subref{fig:hyp1} Distribution of learners' performance before and after first learning activity.\subref{fig:hyp1_2} Comparison of performance statistics before and after learning activity.}
%\label{fig:assessments}
\end{center}
\vspace{-0.3in}
\end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=4in, height=!]{Hyp1_fig.png}
% \caption{Distribution of learners' performance before and after intervention.}
% \label{fig:hyp1}
% \end{figure}

Fig.~\ref{fig:hyp1_2} further summarizes the performance measure in terms of different statistical measures: mean, and median across different groups of learners (refer to Sec.~\ref{sec:data} for details of learner grouping). It is clear from the figure that the performance of the learners on word-image association increases with intervention via the application. %This increase is more prominent in group B students than those in the group A. 

To test if this increase is statistically significant, we perform the t-test for means and non-parametric Kolmogorov-Smirnov test which were described in Sec.~\ref{sec:model}. Both the tests have rejected the null hypothesis and find the difference to be statistically significant (p-values of $2.91\times10^{-57}$ and $2.14\times10^{-46}$ respectively which are rejected with a significance level of $0.1$). 

\subsubsection{Hypothesis 2}
We now move to the next research question of Sec.~\ref{sec:hyp}. The second hypothesis states that the performance of learners is higher for learners in the experimental group than the control group. This question is answered individually for every vocabulary word (concept). To answer this question, we set $G_1$ to be the set of assessment responses of all learners that belong to the control group for the particular vocabulary word (Group B learners for words in word set $X$, and vice versa), and $G_2$ to be the set of assessment responses of all learners that belong to the experimental group for the particular vocabulary word (Group A learners for words in word set $X$, and vice versa). 

\begin{figure}
\centering
\includegraphics[width = 3.5in, height=!]{WordQueue.png}
\caption{Effect of $\eta$ and $\tau$.}
\label{fig:word_queue}
\end{figure}

Clearly, due to the limited pilot study duration, not all vocabulary words have the required information to answer this question. Fig.~\ref{fig:word_queue} shows the number of words with available information with varying parameters of $\tau$ and $\eta$. While there are several words for which we can answer the question if we reduce $\eta$ and/or $\tau$, that would result in a lower confidence in the results. Hence, we pick $\tau=3$ and $\eta=10$, giving a total of $K=19$ vocabulary words with available information for further analysis.

Fig.~\ref{fig:hyp2} compares the average performance of learners in experimental and control groups. As the figure shows, the performance on word-image association test increases among experimental group in almost all the concepts (except \textit{champion} for which it remains almost same).  

\begin{figure}
\centering
\includegraphics[width = 4in, height=!]{Hyp2_Fig.png}
\caption{Performance comparison between experimental and control groups across multiple learning concepts.}
\label{fig:hyp2}
\end{figure}

To test if this increase is statistically significant, we perform the t-test for means and non-parametric Kolmogorov-Smirnov test (KS test) which were described in Sec.~\ref{sec:model}. The results of the tests are in Table~\ref{table:p-vals}. From the table, we can observe that among the learning concepts, $84.2\%$ of the concepts ($16$ out of $19$) reject the null hypothesis when the t-test of means is considered implying that there has been a statistically significant improvement in learner performance on word-image acquisition for these concepts due to the interventions by the tutor-powered application. When the stricter non-parametric KS test is considered, we see $73.68\%$ of the concepts ($14$ out of $19$) rejecting the null hypothesis, which is still a high numbers of concepts. On further analysis, one can also observe that the few concepts/vocabulary words whose difference is not statistically significant are the ones where the control group itself has a high performance, thereby making the increase insignificant. On the other hand, the concepts where the control group was performing low, such as \emph{identical}, \emph{subtraction}, \emph{deciduous}, \emph{pirouette}, and \emph{repair}, the performance increase is highly significant.

\begin{table}[t]
\begin{center}
\caption{p-values of hypothesis testing for different learning concepts (significance level = $0.1$)}
\begin{tabular}{|c||c|c|c|c|}
\hline
Learning concept & t-test p-value & Null Hypothesis & KS-test p-value & Null Hypothesis\\
\hline
\hline
binoculars &0.0059 & Reject&  0.1009& Accept\\
\hline
career & 0.044& Reject& 0.0254    & Reject\\
\hline
champion & 0.492& Accept& 0.6275    & Accept\\
\hline
conflict & 0.002& Reject& 0.0088    &Reject\\
\hline
deciduous & 2.07$\times10^{-13}$& Reject& 1.76$\times10^{-11}$    &Reject\\
\hline
dozen & 0.00023 & Reject& 0.0021    &Reject\\
\hline
half & 0.006& Reject& 0.0089    &Reject\\ 
\hline
hibernate & 0.205& Accept& 0.3369    & Accept\\
\hline
identical & 3.796$\times10^{-09}$& Reject& 2.72$\times10^{-06}$   &Reject\\
\hline
insect & 0.504& Accept& 0.2066    & Accept\\
\hline
measure & 0.029& Reject& 0.0781    & Reject\\
\hline
octagon & 0.017& Reject& 0.0754    & Reject\\
\hline
pirouette & 3.65$\times10^{-06}$& Reject&2.83$\times10^{-07}$  &Reject\\
\hline
prickly & 0.007& Reject&0.0042    &Reject\\
\hline
repair & 1.96$\times10^{-07}$& Reject&3.85$\times10^{-08}$    &Reject\\
\hline
sculpture & 0.002& Reject&0.0004    &Reject\\
\hline
subtraction & 0.002& Reject&0.0002    &Reject\\
\hline
tool & 0.075& Reject&0.0259    & Reject\\
\hline
veterinarian &0.056 & Reject&0.1206& Accept\\
\hline
\end{tabular}
\end{center}
\label{table:p-vals}
\end{table}

